Towards the Integration of an Intuitionistic First-Order Prover into Coq

An efficient intuitionistic first-order prover integrated into Coq is useful to replay proofs found by external automated theorem provers. We propose a two-phase approach: An intuitionistic prover generates a certificate based on the matrix characterization of intuitionistic first-order logic; the certificate is then translated into a sequent-style proof.

==> eptcsdata.tex <==
\providecommand{\firstpage}{30}
\providecommand{\publicationstatus}{J.C. Blanchette and C. Kaliszyk:\\
Hammers for Type Theories (HaTT'16)\\
EPTCS 210, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.210.6}{10.4204/EPTCS.210.6}}


==> header.tex <==
\makeatletter

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{amsmath,amssymb}
\usepackage{hyperref} %hidelink would make ugly border away
%\usepackage{ifdraft}
%\usepackage{natbib}

%\usepackage{parskip}
\setlength{\parindent}{1em}

\usepackage{xcolor}
%\usepackage[toc,xindy]{glossaries} %https://en.wikibooks.org/wiki/LaTeX/Glossary
%\usepackage{geometry}
%\tolerance=300
%\hypersetup{final}

%\definecolor{linkColor}{RGB}{200,230,255}
%\hypersetup{
%  allbordercolors    = linkColor %Colour of internal links
%}

\usepackage[english]{babel}
%\addto\extrasenglish{\renewcommand{\chapterautorefname}{Chapter}}%make the "chapter XX" in autoref capitalized 
%\addto\extrasenglish{\renewcommand{\sectionautorefname}{Section}}%make the "chapter XX" in autoref capitalized 


%\newcommand{\dragons}{{\includegraphics[width=6cm,draft=false]{dragons.PNG}}\\}


\usepackage{xspace} %no space after math
%\usepackage{xparse} %for non-italic theorem
%\usepackage{tikz}          
%\usetikzlibrary{arrows,decorations,arrows.meta}
%\usetikzlibrary{calc} %middle of two notes in chpARS


\def\sectionautorefname{Section}

%\usepackage{graphicx} %dashed down-arrow

%\usepackage{subcaption} %subfigures

\usepackage{ifdraft} %for todos and draft mode
\ifdraft{%
	%\usepackage{setspace}
	%\doublespacing
    \usepackage{todonotes}}{ % draft with TODOs
    \usepackage[disable]{todonotes} % final without TODOs
}


\newcommand{\todoi}[1]{\todo[inline]{#1}}


\usepackage{ntheorem}
\newtheorem{exmp}{Example}


\input{notation}

\makeatother


==> notation.tex <==
%general
\newcommand{\trans}[1]{\mathrel{{#1}^{*}}}
\newcommand{\transRel}[1]{\mathrel{\stackrel{*}{#1}}}


\newcommand{\N}{\mathbb{N}}

\newcommand{\defined}[1]{\textbf{#1}\index{#1}}

%ARS
\DeclareMathOperator{\redRel}{\rightarrow}
\newcommand{\red}{\mathrel{\rightarrow}}
\newcommand{\revRed}{\mathrel{\leftarrow}}
\newcommand{\redP}[1]{\mathrel{\stackrel{#1}{\red}}}
\newcommand{\revRedP}[1]{\mathrel{\stackrel{#1}{\revRed}}}
\newcommand{\redC}{\transRel{\red}}
\newcommand{\revRedC}{\transRel{\revRed}}
\newcommand{\redEq}{\mathrel{\stackrel{*}{\leftrightarrow}}}
\newcommand{\evalsP}[3]{{#2}\Downarrow^{#1}{#3}}
\newcommand{\evals}[2]{{#1}\Downarrow{#2}}



